Learning Task Priorities from Demonstrations

Bimanual operations in humanoids offer the possibility to carry out more than one manipulation task at the same time, which in turn introduces the problem of task prioritization. We address this problem from a learning from demonstration perspective, by extending the Task-Parameterized Gaussian Mixture Model (TP-GMM) to Jacobian and null space structures. The proposed approach is tested on bimanual skills but can be applied in any scenario where the prioritization between potentially conflicting tasks needs to be learned. We evaluate the proposed framework in: two different tasks with humanoids requiring the learning of priorities and a loco-manipulation scenario, showing that the approach can be exploited to learn the prioritization of multiple tasks in parallel.

==> sections/JointTaskPriorityConstraints.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% IV
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Learning configuration space and priority constraints}
\label{sec:combiningConstraints}
%%JS: Here, I'm pasting the content of Sylvain's tutorial directly, with some very minor modifications.

The previous section considered the case in which the task parameters were related to object poses in operational space. However, TP-GMM is not limited to this parameterization and can be applied to other forms of locally linear transformations or projections. We will now show that the consideration of non-square $\mb{A}_{t,j}$ matrices allows for the combination of soft constraints in both configuration and operational spaces (through Jacobian operators), see also \cite{Calinon09AR} for a preliminary work in this direction. 
%With a preliminary model of task-parameterized movements, we explored in \cite{Calinon09AR} how a similar approach could be used to simultaneously learn constraints in joint space and task space.

%Another important and challenging category of applications includes the problems requiring priority constraints \cite{Towell10,Lober14,Hak12b,Wrede13}.
%Such
In addition, priority constraints can be learned and encoded within a TP-GMM from an initial set of task hierarchies given as potential candidates to describe the observed skill. The probabilistic encoding is here exploited to discover, from a statistical analysis of the demonstrations, in which manner subtasks are prioritized. 
The different frames correspond in this case to various candidate subspace projections of the movement, with statistical information extracted from the different projections. 
Note that the problem of learning and controlling a robot by considering task priorities can be tackled both at kinematic or dynamic levels. We will define it here at a kinematic level with a robot controlled in joint velocity, but the presented techniques also apply to torque controllers.

%\begin{table*}%[!t]
%\begin{mdframed}
%\caption{Task parameters as candidate projection operators (with affine transformations defined by $\mb{A}_{t,j}$ and $\mb{b}_{t,j}$).}
%\label{tab:Ab}
%\begin{minipage}{12cm}
%\begin{align}
%  \mb{\hat{q}}^{(j)}_{t,i} &=
%  \mb{I} 
%  & \mb{\mu}^{(j)}_i &+ 
%  \mb{0} 
%  \label{eq:Ab_q}\\
%	%
%	\mb{\hat{q}}^{(j)}_{t,i} &=
%	\mb{J}^\psin\!(\mb{q}_{t-1})
%	& \mb{\mu}^{(j)}_i &+
%	\mb{q}_{t-1} - \mb{J}^\psin\!(\mb{q}_{t-1}) \mb{x}_{t-1} 
%	\label{eq:Ab_x}\\
%	%
%	\mb{\hat{q}}^{(j)}_{t,i} &=
%  \mb{J}^\psin\!(\mb{q}_{t-1}) \mb{A}^\ty{O}_t 
%  & \mb{\mu}^{(j)}_i &+
%	\mb{q}_{t-1} + \mb{J}^\psin\!(\mb{q}_{t-1}) \big[ \mb{b}^\ty{O}_t - \mb{x}_{t-1}\big] 
%	\label{eq:Ab_xo}\\
%	%
%	\mb{\hat{q}}^{(j)}_{t,i} &=
%	\mb{N}\!(\mb{q}_{t-1})
%  & \mb{\mu}^{(j)}_i &+
%	\mb{J}^\psin\!(\mb{q}_{t-1}) \mb{J}\!(\mb{q}_{t-1}) \mb{q}_{t-1} 
%	\label{eq:Ab_Nq}\\
%	%
%	\mb{\hat{q}}^{(j)}_{t,i} &=
%  \mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!\!(\mb{q}_{t-1}) 
%  & \mb{\mu}^{(j)}_i &+
%	\mb{q}_{t-1} - \mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!\!(\mb{q}_{t-1}) \; \mb{x}_{t-1} 
%	\label{eq:Ab_Nx}\\
%	%
%	\mb{\hat{q}}^{(j)}_{t,i} &=
%  \underbrace{\mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!\!(\mb{q}_{t-1}) \mb{A}^\ty{O}_t}_{\mb{A}_{t,j}}  
%  & \mb{\mu}^{(j)}_i &+
%	\underbrace{\mb{q}_{t-1} \!+\! \mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!\!(\mb{q}_{t-1}) \big[ \mb{b}^\ty{O}_t \!-\! \mb{x}_{t-1}\big] }_{\mb{b}_{t,j}} ,
%	\label{eq:Ab_Nxo}
%\end{align}
%\end{minipage}
%\end{mdframed}
%\end{table*}

\subsection{Learning soft constraints in both configuration and operational spaces}
\label{subsec:combConstraints}

%For a controller handling constraints both in configuration and operational spaces, some of the most common candidate projection operators are presented in Table \ref{tab:Ab}, covering a very wide range of robotics applications.
We first recall that forward and differential kinematics are computed with
\begin{equation}
	\!\mb{x}_t \!=\! f(\mb{q}_t)
	\!\iff\!
	\mb{\dot{x}}_t \!=\! \frac{\partial\mb{x}_t}{\partial t}
	= \frac{\partial f(\mb{q}_t)}{\partial\mb{q}_t} \; \frac{\partial\mb{q}_t}{\partial t} =
	\mb{J}(\mb{q}_t) \; \mb{\dot{q}}_t,
	\label{eq:FKJacobianDef}
\end{equation}
where $\mb{x}_t$, $\mb{\dot{x}}_t$ represent a link pose and velocity (typically the end-effector), $\mb{q}_t = \left[q_{t,1} \>\hdots\> q_{t,N_q}\right]^\trsp$, $\mb{\dot{q}}_t$ are the vectors of joint positions and velocities for a robot with $N_q$ DOFs and $\mb{J}(\mb{q}_t)$ is a Jacobian matrix.

Inverse kinematics is most commonly achieved by minimizing the $L_2$-norm of the residuals
%
\begin{equation}
	\mb{\hat{\dot{\mb{q}}}} = \arg\underset{\mb{\dot{q}}}{\min} {\|\mb{\dot{x}}-\mb{J}\mb{\dot{q}}\|}_2 = \arg\underset{\mb{\dot{q}}}{\min} {(\mb{\dot{x}}-\mb{J}\mb{\dot{q}})}^\trsp\!(\mb{\dot{x}}-\mb{J}\mb{\dot{q}}),
	\label{eq:IKoptimization}
\end{equation}
by dropping the dependencies on $\mb{q}$ and $t$ in the notation. The general least norm inverse kinematics solution is  given by
%
\begin{equation}
	\mb{\hat{\dot{\mb{q}}}} = \mb{J}^\psin \mb{\dot{x}} + \mb{N} \mb{\dot{q}}_0,%g(\mb{q}),
	\label{eq:generalIKsol}
\end{equation}
with $\mb{J}^\psin=\mb{J}^\trsp {\big(\mb{J}\mb{J}^\trsp\big)}^{-1}$ the right pseudoinverse of the Jacobian, $\mb{N} = \mb{I} - \mb{J}^\psin \mb{J}$ the null-space projection operator, and $\mb{\dot{q}}_0$ a secondary objective that will not affect the principal $L_2$-norm minimization objective.

In operational space control, as tasks can be defined at the level of position and orientation, the Jacobian matrix is typically comprised of two block matrices
\begin{equation}
	\mb{\dot{x}}= \mb{J} \>\mb{\dot{q}}
	\iff
	\left[\begin{matrix} \mb{\dot{p}} \\ \mb{\omega}	\end{matrix}\right] = \left[\begin{matrix} \mb{J_p} \\ \mb{J_o} \end{matrix} \right] \mb{\dot{q}},
	\label{eq:Jacobian}
\end{equation}
where $\mb{J}\in\mathbb{R}^{6\times N_q}$ is the geometric Jacobian%\footnote{The geometric Jacobian maps $\mb{\dot{q}}$ to $\mb{\omega}$, while the analytical Jacobian maps $\mb{\dot{q}}$ to the rates of other - minimal - representation of orientation, such as Euler angles \cite{Siciliano09Book}.}.
, consisting of two sub-matrices $\mb{J_p}\in \mathbb{R}^{3\times N_q}$, $\mb{J_o}\in \mathbb{R}^{3\times N_q}$ which map joint velocities to the end-effector linear and angular velocities, $\mb{\dot{p}}\in \mathbb{R}^3$, $\mb{\omega}\in \mathbb{R}^3$.
%% JS: I removed the footnote above to gain some space.

The TP-GMM representation can be extended to task parameters $\{\mb{b}_{t,j},\mb{A}_{t,j}\}_{j=1}^P$ with different dimensionality for each candidate frame $j$ and non-square $\mb{A}_{t,j}$ matrices. %(candidate projections)
In particular, we exploit the kinematic relationships given by \eqref{eq:IKoptimization}, \eqref{eq:generalIKsol} and \eqref{eq:Jacobian} to formulate the task parameters in a way that operational space constraints are projected on configuration space, where Gaussian products are computed. %A wide range of robot skills can be defined in such way., see e.g.\ the possible tasks described in Chapter 6.2.1 of \cite{Antonelli14}.

Table \ref{tab:AbOrient} gives a summary of how these operators are defined for different kinds of constraints. For completeness, we derive in Appendix \ref{app:TPsoftConstraints} some of those operators, with a particular attention on orientation.

\begin{table*}%[!t]
	\begin{mdframed}
		\vspace{0.3cm}
		\caption{Summary of task parameters for candidate projection operators.}
		\label{tab:AbOrient}
		\centering
		\vspace{-0.3cm}
		\begin{minipage}{17.5cm}
			\begin{align}
			\!\!\!\!\!\!\!\!
			&\begin{matrix} \text{\textit{Configuration space constraints}}\\ \text{\textit{ in a fixed frame:}}
			\end{matrix}
			\!\!\! &\mb{\hat{q}}^{(j)}_{t,i} &=
			\mb{I} 
			& \!\!\!\!\!\!\mb{\mu}^{(j)}_i &+ 
			\mb{0} 
			\label{eq:Ab_qTable}\\
			%
			\!\!\!\!\!\!\!\!
			&\begin{matrix} \text{\textit{Absolute position/orientation}} \\ \text{\textit{constraints:}}
			\end{matrix}
			\!\!\! &\mb{\hat{q}}^{(j)}_{t,i} &=
			\mb{J}^\psin\!(\mb{q}_{t-1})
			\left[\begin{matrix}
			\>\> \mb{I} & \mb{0} \\ 
			\>\> \mb{0} & \HRightVec(\mb{\bar{\epsilon}}_{t-1})
			\end{matrix} \right]
			& \!\!\!\!\!\!\mb{\mu}^{(j)}_i & -
			\mb{J}^\psin\!(\mb{q}_{t-1})
			\left[\begin{matrix}
			\mb{x}_{t-1} \\
			\mb{0}	\end{matrix} \right]
			+ \mb{q}_{t-1}
			\label{eq:Ab_xTable}\\
			%
			\!\!\!\!\!\!\!\!
			&\begin{matrix} \text{\textit{Relative position/orientation}} \\ \text{\textit{constraints:}}
			\end{matrix}
			\!\!\! &\mb{\hat{q}}^{(j)}_{t,i} &=
			\mb{J}^\psin\!(\mb{q}_{t-1})
			\left[\begin{matrix}
			\>\> \mb{R}^\ty{O}_t & \mb{0} \\
			\>\> \mb{0} & \HRightVec(\mb{\bar{\epsilon}}_{t-1}) \>\HLeft(\mb{\epsilon}^{\ty{O}}_t) 
			\end{matrix} \right]
			& \!\!\!\!\!\!\mb{\mu}^{(j)}_i &+
			\mb{J}^\psin\!(\mb{q}_{t-1})
			\left[\begin{matrix}
			\mb{x}^\ty{O}_t - \mb{x}_{t-1} \\
			\mb{0}
			\end{matrix} \right] +
			\mb{q}_{t-1}
			\label{eq:Ab_xoTable}\\
			%
			\!\!\!\!\!\!\!\!
			&\begin{matrix}
			\text{\textit{Null-space constraints in}} \\ \text{\textit{configuration space:}}
			\end{matrix}
			\!\!\! &\mb{\hat{q}}^{(j)}_{t,i} &=
			\mb{N}\!(\mb{q}_{t-1})
			& \!\!\!\!\!\!\mb{\mu}^{(j)}_i &+
			\mb{J}^\psin\!(\mb{q}_{t-1}) \mb{J}\!(\mb{q}_{t-1}) \mb{q}_{t-1} 
			\label{eq:Ab_NqTable}\\
			%
			\!\!\!\!\!\!\!\!
			&\begin{matrix} \text{\textit{Absolute position/orientation}} \\ \text{\textit{null-space constraints:}}
			\end{matrix}
			\!\!\! &\mb{\hat{q}}^{(j)}_{t,i} &=
			\mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!(\mb{q}_{t-1})
			\left[\begin{matrix}
			\>\> \mb{I} & \mb{0} \\ 
			\>\> \mb{0} & \HRightVec(\mb{\bar{\epsilon}}_{t-1})
			\end{matrix} \right]
			& \!\!\!\!\!\!\mb{\mu}^{(j)}_i &-
			\mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!\!(\mb{q}_{t-1})
			\left[\begin{matrix}
			\mb{x}_{t-1} \\
			\mb{0}
			\end{matrix} \right] +
			\mb{q}_{t-1} 
			\label{eq:Ab_NxTable}\\
			%
			\!\!\!\!\!\!\!\!
			&\begin{matrix} \text{\textit{Relative position/orientation}} \\ \text{\textit{null-space constraints:}}
			\end{matrix}
			\!\!\! &\mb{\hat{q}}^{(j)}_{t,i} &=
			\underbrace{
				\mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!(\mb{q}_{t-1})
				\left[\begin{matrix}
				\>\> \mb{R}^\ty{O}_t & \mb{0} \\
				\>\> \mb{0} & \HRightVec(\mb{\bar{\epsilon}}_{t-1}) \>\HLeft(\mb{\epsilon}^{\ty{O}}_t) 
				\end{matrix} \right]
			}_{\mb{A}_{t,j}}  
			& \!\!\!\!\!\!\mb{\mu}^{(j)}_i &+
			\underbrace{
				\mb{N}\!(\mb{q}_{t-1}) \mb{\tilde{J}}^{\;\psin}\!\!(\mb{q}_{t-1}) 
				\left[\begin{matrix}
				\mb{x}^\ty{O}_t \!-\! \mb{x}_{t-1}\\
				\mb{0}
				\end{matrix} \right]+
				\mb{q}_{t-1}
			}_{\mb{b}_{t,j}}
			\label{eq:Ab_NxobjTable}
			\end{align}
		\end{minipage}
		\vspace{-0.15cm}
	\end{mdframed}
	\vspace{-0.5cm}
\end{table*}


\subsection{Learning priority constraints}
\label{subsec:priorityConstraints}
TP-GMM provides a principled way to learn and synthesize task priorities from a probabilistic representation of strict candidate hierarchies. We argue that the operational space contains incomplete information for the recognition of tasks that are being executed in parallel, and that the extraction of task constraints can be enriched by combining observations in operational and configuration spaces. This situation is illustrated in Figure \ref{fig:hierarchyConstraints}. In this example, we consider a planar robot that tracks the position and orientation of an object with its end-effector. The top-right graph shows the observed tracking errors in position and orientation spaces collected from four demonstrations. The two observation sets, A and B, show two different interpretations of the error data. Observation set A shows that the dataset could have been generated by a demonstrator who was carefully tracking the orientation of the object, while neglecting the tracking of the position, resulting in poor accuracy in position tracking. Observation set B shows a different interpretation of the same data. It shows that the variability in position tracking was the result of the object being too far away for the robot to track both position and orientation. This illustrative example shows that, by observing the configuration of the robot, we can interpret the error data as an equally accurate tracking of position and orientation with a priority on orientation. Intuitively, we can observe, from the configuration of the robot, that it actually tracks the position as effectively as it can, given the priority constraint. The proposed approach formalizes this problem by representing priority constraints as candidate projections in a probabilistic task-parameterized model. 

%%A statistical analysis of observed operational space movements is performed through their re-projection in operational space, by considering different candidate hierarchies that could have been responsible for the generation of the observed behavior.
%A statistical analysis of the observed operational space movements is performed, by considering the different candidate hierarchies that could have been responsible for the generation of the observed behavior.
%This analysis results in different importances that are represented by weights associated with each candidate hierarchy. It consequently follows that new movements can be synthesized through a \textit{soft weighting of strict hierarchies}, a combination of two approaches that were previously used independently. Each candidate hierarchy thus provides a potential inverse kinematics solution with an associated importance, in a similar fashion to the description in Section \ref{subsec:combConstraints} for operational and configuration space constraints. We assume here that the candidate task structures are given and that the kinematic model of the robot is known, i.e., that the Jacobian of each task is available.  

\begin{figure}
	\centering
%	\includegraphics[width=0.8\textwidth]{figures/hierarchyConstraints01}
%	\includegraphics[width=\columnwidth]{figures/hierarchyConstraints01vertical}
%	\includegraphics[width=\columnwidth]{figures/hierarchyConstraints01vertical_compact}
	\includegraphics[width=\columnwidth]{figures/hierarchyConstraints01vertical_compact_legend}
	\caption{Importance of the configuration space when observing a movement for the automatic extraction of hierarchy constraints. A planar robot tracks the position and orientation of an object. The top-right graph shows the tracking errors. Observation sets A and B show different options for the underlying source of the tracking errors: neglecting position tracking (A), and tracking orientation as a priority with position as a secondary goal (B).
%Illustration of the importance of the configuration space when observing a movement for the automatic extraction of hierarchy constraints. The task consists of controlling the vertical position and the orientation of the end-effector such that it matches the position and orientation of an object. Four demonstrations are provided, depicted in blue, red, yellow and purple colors. The left graphs shows the observed tracking errors in position and orientation spaces collected for the four demonstrations. The right part of the figure shows two different interpretations of the data. The top graphs show the dataset could have been generated by a demonstrator who was carefully tracking the orientation of the object, while neglecting the tracking of the position, resulting in poor accuracy in position tracking. The bottom graphs show a different interpretation of the same data. Here, it shows that the variability in position tracking was the result of the object being too far away for the robot to track both position and orientation. This illustrative example shows that by observing the configuration of the robot, we can interpret the error data as an equally accurate tracking of position and orientation with a priority on orientation. Intuitively, we can observe from the configuration of the robot that it actually tracks the position as effectively as it can given the priority constraint. The proposed approach formalizes this problem by representing priority constraints as candidate projections in a probabilistic task-parameterized model. 
	}
	\label{fig:hierarchyConstraints}
\end{figure}

%\subsection*{Introductory example: planar robot with position and orientation tasks}

Let us consider again the planar robot with position and orientation tasks of Fig.\ \ref{fig:hierarchyConstraints}. If the two tasks in operational space are defined by desired Cartesian velocities $\mb{\dot{x}}_1$ and $\mb{\dot{x}}_2$, \eqref{eq:generalIKsol} can be exploited to explicitly define a strict priority of one task over the other when computing inverse kinematics, i.e.,
\begin{equation}
\mb{\hat{\dot{\mb{q}}}} 
= \mb{J}_{\!1}^\psin \; \mb{\dot{x}}_1 + \mb{N}_{\!1} \mb{J}_{\!2}^\psin \; \mb{\dot{x}}_2 \\
%&= \mb{J}_1^\trsp {(\mb{J}_1\mb{J}_1^\trsp)}^{-1} \; \mb{\dot{x}}_1 + 
%\left(\mb{I} - \mb{J}_1^\trsp {(\mb{J}_1\mb{J}_1^\trsp)}^{-1} \mb{J}_1\right) \; 
%\mb{J}_2^\trsp{(\mb{J}_2\mb{J}_2^\trsp)}^{-1} \; \mb{\dot{x}}_2 \\
= \left[\mb{J}_{\!1}^\psin \quad \mb{N}_{\!1}\mb{J}_{\!2}^\psin \right] 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right].
\label{eq:strictPriorityx1}
\end{equation}

The resulting velocity in operational space is given by
\begin{align}
\left[\begin{matrix} \mb{\hat{\dot{x}}}_1 \\ \mb{\hat{\dot{x}}}_2 \end{matrix}\right] 
&= \left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right] \mb{\hat{\dot{\mb{q}}}} = \left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right]
\left[\mb{J}_{\!1}^\psin \quad \mb{N}_{\!1}\mb{J}_{\!2}^\psin \right] 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right] \nonumber\\
%&= \left[\begin{matrix} \mb{J}_1\mb{J}_1^\psin & \mb{J}_1\mb{N}_1\mb{J}_2^\psin \\
%\mb{J}_2\mb{J}_1^\psin & \mb{J}_2\mb{N}_1\mb{J}_2^\psin
%\end{matrix}
%\right] 
%\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right] \nonumber\\
&\approx \left[\begin{matrix} \mb{I} & \mb{0} \\
\mb{J}_{\!2}\mb{J}_{\!1}^\psin & \mb{J}_{\!2}\mb{N}_{\!1}\mb{J}_{\!2}^\psin
\end{matrix}
\right] 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right],
\label{eq:Task1HierarchyOp}
\end{align}
%
where the final expression comes from the definition of the pseudoinverse and null-space projection matrices.
Similarly, if
\begin{equation}
\mb{\hat{\dot{\mb{q}}}} 
= \mb{J}_{\!2}^\psin \; \mb{\dot{x}}_2 + \mb{N}_{\!2} \mb{J}_{\!1}^\psin \; \mb{\dot{x}}_1 \\
= \left[\mb{N}_{\!2}\mb{J}_{\!1}^\psin \quad \mb{J}_{\!2}^\psin\right] 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right],
\label{eq:strictPriorityx2}
\end{equation}
%
the resulting velocity in operational space is given by
%
\begin{equation}
\left[\begin{matrix} \mb{\hat{\dot{x}}}_1 \\ \mb{\hat{\dot{x}}}_2 \end{matrix}\right] 
%= \left[\begin{matrix} \mb{J}_1 \\ \mb{J}_2 \end{matrix}\right] 
%\left[\mb{N}_2\mb{J}_1^\psin \quad \mb{J}_2^\psin \right]  
%\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right] \nonumber\\
%&= \left[\begin{matrix} \mb{J}_1\mb{N}_2\mb{J}_1^\psin & \mb{J}_1\mb{J}_2^\psin \\
%\mb{J}_2\mb{N}_2\mb{J}_1^\psin & \mb{J}_2\mb{J}_2^\psin 
%\end{matrix}
%\right] 
%\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right] \nonumber\\
\approx \left[\begin{matrix} \mb{J}_{\!1}\mb{N}_{\!2}\mb{J}_{\!1}^\psin & \mb{J}_{\!1}\mb{J}_{\!2}^\psin \\
\mb{0} & \mb{I}
\end{matrix}
\right] 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right].
\label{eq:Task2HierarchyOp}
\end{equation}

%\begin{figure}
%	\centering
%	\includegraphics[width=.48\textwidth]{figures/demoIK_hierarchyExtraction02d}
%	\caption{
%Evaluation of two candidate hierarchies from the dataset in Fig.\ \ref{fig:hierarchyConstraints} (left). The left graphs correspond to the candidate hierarchy in which position has priority over orientation \eqref{eq:Task1HierarchyOp}, while the right graphs show the case of priority on orientation \eqref{eq:Task2HierarchyOp}.
%	}
%	\label{fig:hierarchyConstraints2}
%\end{figure}

\begin{figure}
	\begin{subfigure}{0.47\columnwidth}
		\centering
		\includegraphics[width=1.0\columnwidth]{figures/toyExample_priorityOrient.pdf}
		\caption{}
		\label{fig:hierarchyConstraints2Orient}
	\end{subfigure}%
	\hspace{4mm}
	\begin{subfigure}{0.47\columnwidth}
		\centering
		\vspace{0.4mm}	% some alignment because images aren't exactly the same size
		\includegraphics[width=0.835\columnwidth]{figures/toyExample_priorityPos.pdf}
		\caption{}
		\label{fig:hierarchyConstraints2Pos}
	\end{subfigure}
	\vspace{0.2cm}
	\caption{Projection of task space errors by considering two different candidate hierarchies. \textbf{(a)} Demonstrated priority on orientation (Fig. \ref{fig:hierarchyConstraints}, Observation set B) \textbf{(b)} Demonstrated priority on position (Fig. \ref{fig:hierarchyConstraints3}).}
	\label{fig:hierarchyConstraints2}
\end{figure}

\begin{figure}
	\centering
	%	\includegraphics[width=.41\textwidth]{figures/demoIK_hierarchyExtraction02e}\\
	\includegraphics[width=.41\textwidth]{figures/demoIK_hierarchyExtraction02e_compact}
	%	\includegraphics[width=.48\textwidth]{figures/demoIK_hierarchyExtraction02f}
	\caption{Evaluation of candidate hierarchies for a new dataset: priority on position tracking with secondary task of tracking orientation.}
	\label{fig:hierarchyConstraints3}
\end{figure}

For a controller generating operational space movements $\left[ \mb{\dot{x}}^\trsp_1 \quad \mb{\dot{x}}^\trsp_2\right]^\trsp$, the projection operators in \eqref{eq:Task1HierarchyOp} and \eqref{eq:Task2HierarchyOp} can be used to evaluate which hierarchy is responsible for the observed movement. %The example in Fig. \ref{fig:hierarchyConstraints} corresponds to a case where the two tasks are the tracking of position and orientation references. %Let us assume that $\mb{\dot{x}}_1$ and $\mb{\dot{x}}_2$ correspond to the position and orientation tasks, respectively.
We apply operators \eqref{eq:Task1HierarchyOp} and \eqref{eq:Task2HierarchyOp} to the dataset obtained in Fig.\ \ref{fig:hierarchyConstraints} (top-right), which corresponds to the  position and orientation tracking errors in four demonstrations, $e_y$ and $e_o$. Figure \ref{fig:hierarchyConstraints2Orient} shows the projected datapoints, with the corresponding variability, for the two candidate hierarchies. We observe that the projected data exhibits low variability for the hierarchy that has orientation as a priority over position, indicating that the data was generated by a controller whose main priority was orientation tracking. Figure \ref{fig:hierarchyConstraints2Pos} shows that we can reach a similar observation for a new dataset with priority on position and orientation as a secondary goal (Fig.\ \ref{fig:hierarchyConstraints3}). %shows that for such a scenario the distribution of the datapoints obtained using \eqref{eq:Task1HierarchyOp} has a notably lower variance compared to that obtained with \eqref{eq:Task2HierarchyOp}.

In this simple example, the analysis of the variance of the projected data provides a way of assigning importance to each candidate hierarchy. The same approach can be employed to learn the orchestration of structures in more complex ways, with changes of hierarchies along the task and with richer parallel organization of task structures. We take advantage of this model to compute full precision matrices that are associated with each candidate projection operator. It consequently follows that new movements can be synthesized through a \textit{soft weighting of strict hierarchies}, a combination of two approaches that were previously used independently. We assume here that the candidate task structures are given and that the kinematic model of the robot is known, i.e., that the Jacobian of each task is available.  


\subsection{Soft weighting of strict hierarchies}
\label{subsec:softWeighting}
If we redefine the optimization problem \eqref{eq:IKoptimization} as
%
\begin{equation*}
\mb{\hat{\dot{\mb{q}}}}  
= \arg\underset{\mb{\dot{q}}}{\min}\; {(\mb{\hat{\dot{x}}}-\mb{J}\mb{\dot{q}})}^\trsp \mb{W} (\mb{\hat{\dot{x}}}-\mb{J}\mb{\dot{q}}),
\end{equation*}
%
the inverse kinematics solution is given by the weighted pseudoinverse
%
\begin{equation*}
\mb{\hat{\dot{\mb{q}}}}
=
{(\mb{J}^\trsp \mb{W}\mb{J})}^{-1}\mb{J}^\trsp \mb{W} \, \mb{\hat{\dot{x}}}  .
\end{equation*}
%
By assigning two importance weights $w_1$ and $w_2$ to the two tasks $\mb{\dot{x}}_1$ and $\mb{\dot{x}}_2$, the above formulation can be used to compute a solution that corresponds to a soft weighting of the tasks, as opposed to a strict hierarchy such as \eqref{eq:strictPriorityx1}, \eqref{eq:strictPriorityx2}. Namely:
%
\begin{equation*}
\mb{\hat{\dot{\mb{q}}}}
=
{\left({\left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right]}^\trsp\!\! 
	\left[\begin{matrix} w_1\mb{I} & \mb{0} \\ \mb{0} & w_2\mb{I} \end{matrix}\right]\!\!\!
	\left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right]\right)}^{\!\!-1}
{\left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right]}^\trsp \!\!
\left[\begin{matrix} w_1\mb{I} & \mb{0} \\ \mb{0} & w_2\mb{I} \end{matrix}\right]\!\!\! 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right] .
%\mb{\dot{x}} = \left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right]
%\;,\;
%\mb{J} = \left[\begin{matrix} \mb{J}_1 \\ \mb{J}_2 \end{matrix}\right]
%\;,\;
%\mb{W} = \left[\begin{matrix} w_1\mb{I} & 0 \\ 0 & w_2\mb{I} \end{matrix}\right] .
\end{equation*}

Similarly, with precision matrices $\mb{\Gamma}_1$ and $\mb{\Gamma}_2$, we get
%
\begin{align*}
\mb{\hat{\dot{\mb{q}}}}
&=
{\left({\left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right]}^\trsp 
	\left[\begin{matrix} \mb{\Gamma}_1 & \mb{0} \\ \mb{0} & \mb{\Gamma}_2 \end{matrix}\right]
	\left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right]\right)}^{\!\!-1}
{\left[\begin{matrix} \mb{J}_{\!1} \\ \mb{J}_{\!2} \end{matrix}\right]}^\trsp 
\left[\begin{matrix} \mb{\Gamma}_1 & \mb{0} \\ \mb{0} & \mb{\Gamma}_2 \end{matrix}\right] 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \mb{\dot{x}}_2 \end{matrix}\right] \\
&=
{\left(\mb{J}_{\!1}^\trsp\mb{\Gamma}_1\mb{J}_{\!1} + \mb{J}_{\!2}^\trsp\mb{\Gamma}_2\mb{J}_2\right)}^{-1}
\left(\mb{J}_{\!1}^\trsp\mb{\Gamma}_1\mb{\dot{x}}_1 + \mb{J}_{\!2}^\trsp\mb{\Gamma}_2\mb{\dot{x}}_2\right),
\end{align*}
%
which is analogous to a product of linearly transformed Gaussians with centers $\mb{\dot{x}}_1$ and $\mb{\dot{x}}_2$, precision matrices $\mb{\Gamma}_1$ and $\mb{\Gamma}_2$, and projection operators $\mb{J}_{\!1}^\trsp$ and $\mb{J}_{\!2}^\trsp$.

The most common approaches for controlling tasks of different priorities are either based on strict hierarchies \cite{Wrede13,Saveriano15,Towell10,Hak12b}, or soft weighting of tasks \cite{Moro13,Dehio15,Modugno16,Lober15}. We propose a richer alternative based on a \textit{soft weighting of strict hierarchies}, gathering the best of the two approaches. 
%
%We define the two candidate projection operators $\mb{A}_1\!=\!\left[\mb{J}_1^\psin \quad \mb{N}_1\mb{J}_2^\psin \right]$ and $\mb{A}_2\!=\!\left[\mb{N}_2\mb{J}_1^\psin \quad \mb{J}_1^\psin \right]$, representing respectively a priority of $\mb{\dot{x}}_1$ over $\mb{\dot{x}}_2$, and a priority of $\mb{\dot{x}}_2$ over $\mb{\dot{x}}_1$. 
%
For the two task case, we define the two candidate hierarchies
%
\begin{equation}
\mb{A}_1 = \left[\mb{J}_1^\psin \quad \mb{N}_1\mb{J}_2^\psin \right] 
,\quad
\mb{A}_2 = \left[\mb{N}_2\mb{J}_1^\psin \quad \mb{J}_2^\psin \right]
,
\label{eq:TaskParametersNoObject}
\end{equation}
%
representing respectively a priority of $\mb{\dot{x}}_1$ over $\mb{\dot{x}}_2$, and a priority of $\mb{\dot{x}}_2$ over $\mb{\dot{x}}_1$. 
By using a task-parameterized representation% (here, with a single Gaussian instead of a GMM)
, a statistical analysis of the observed data is achieved with the candidate projections $\left[\mb{J}^\trsp_1 \>\> \mb{J}^\trsp_2\right]^\trsp\!\!\mb{A}_1$ and $\left[\mb{J}^\trsp_1 \>\> \mb{J}^\trsp_2\right]^\trsp\!\!\mb{A}_2$, as in \eqref{eq:Task1HierarchyOp} and \eqref{eq:Task2HierarchyOp}, providing precision matrices % $\mb{\tilde{\Gamma}}_1$ and $\mb{\tilde{\Gamma}}_2$
in operational space that are learned from observations. 
%
These can then be used to generate behaviors in new configurations, with a weighting of candidate hierarchies similar to the demonstrations. If we consider two Gaussians, with centers $\mb{\mu}^{(1)}$, $\mb{\mu}^{(2)}$ and precision matrices $\mb{\tilde{\Gamma}}_1$ and $\mb{\tilde{\Gamma}}_2$ (inverses of the covariance matrices), estimated from observations of $\mb{\dot{x}}^{(1)} = \left[\mb{\dot{x}}^{(1)\;\trsp}_1 \>\> \mb{\dot{x}}^{(1)\;\trsp}_2\right]^\trsp$ and $\mb{\dot{x}}^{(2)} = \left[\mb{\dot{x}}^{(2)\;\trsp}_1 \>\> \mb{\dot{x}}^{(2)\;\trsp}_2\right]^\trsp$ (superscripts denote candidate hierarchies, subscripts denote task velocities as in \eqref{eq:Task1HierarchyOp},\eqref{eq:Task2HierarchyOp}), this is achieved by considering the controller
%
%where $\mb{\dot{x}}^{(1)} = \left[\mb{\dot{x}}^{(1)\;\trsp}_1 \>\> \mb{\dot{x}}^{(1)\;\trsp}_2\right]^\trsp$ and $\mb{\dot{x}}^{(2)} = \left[\mb{\dot{x}}^{(2)\;\trsp}_1 \>\> \mb{\dot{x}}^{(2)\;\trsp}_2\right]^\trsp$ are the centers of the Gaussians encoding the priority on tasks 1 and 2 as operational space velocities or tracking errors, estimated from projections \eqref{eq:Task1HierarchyOp}-\eqref{eq:Task2HierarchyOp}, where $\mb{\tilde{\Gamma}}_1$ and $\mb{\tilde{\Gamma}}_2$ are the inverses of the covariance matrices.
%
\begin{equation}
\mb{\hat{\dot{\mb{q}}}}
=
\!{\left(\!\mb{A}_1\mb{\tilde{\Gamma}}_1\mb{A}^\trsp_1 \!+\! \mb{A}_2\mb{\tilde{\Gamma}}_2\mb{A}_2^\trsp\right)}^{\!\!-1}
\!\!\!\left(\!\mb{A}_1\mb{\tilde{\Gamma}}_1\mb{\mu}^{(1)} \!+\! \mb{A}_2\mb{\tilde{\Gamma}}_2\mb{\mu}^{(2)}\right)\!.
\label{eq:controllerWeightingStrictHierarchies}
\end{equation}
%

%This can be used co-jointly with a standard definition of task parameters as object-related movement. For two objects with orientations $\mb{R}^\ty{O}_1, \mb{R}^\ty{O}_2$ and positions $\mb{x}^\ty{O}_1, \mb{x}^\ty{O}_2$, this can for example be achieved by defining
%\begin{align}
%\mb{A}_1 = \left[\mb{J}_1^\psin \quad \mb{N}_1\mb{J}_2^\psin \right] \left[\begin{matrix} \mb{R}^\ty{O}_1 \\ \mb{R}^\ty{O}_2 \end{matrix}\right]\!\!
%,&\>\>
%\mb{b}_1 = \left[\mb{J}_1^\psin \quad \mb{N}_1\mb{J}_2^\psin \right] \left[\begin{matrix} \mb{x}^\ty{O}_1 - \mb{x}_1 \\ \mb{x}^\ty{O}_2 - \mb{x}_2 \end{matrix}\right]
%,\nonumber\\
%\mb{A}_2 = \left[\mb{N}_2\mb{J}_1^\psin \quad \mb{J}_2^\psin \right] \left[\begin{matrix} \mb{R}^\ty{O}_1 \\ \mb{R}^\ty{O}_2 \end{matrix}\right]\!\!
%,&\>\>
%\mb{b}_2 = \left[\mb{N}_2\mb{J}_1^\psin \quad \mb{J}_2^\psin \right] \left[\begin{matrix} \mb{x}^\ty{O}_1 - \mb{x}_1 \\ \mb{x}^\ty{O}_2 - \mb{x}_2 \end{matrix}\right].
%\label{eq:TaskParametersWithObjectTracking}
%\end{align}

This can be used co-jointly with a standard definition of task parameters as object-related movement. For two objects with positions $\mb{x}^\ty{O}_1, \mb{x}^\ty{O}_2$, this is achieved by defining
%
\begin{align}
\mb{A}_1 = \left[\mb{J}_1^\psin \quad \mb{N}_1\mb{J}_2^\psin \right] 
,&\>\>
\mb{b}_1 = \mb{A}_1 \left[\begin{matrix} \mb{x}^\ty{O}_1 - \mb{x}_1 \\ \mb{x}^\ty{O}_2 - \mb{x}_2 \end{matrix}\right]
,\nonumber\\
\mb{A}_2 = \left[\mb{N}_2\mb{J}_1^\psin \quad \mb{J}_2^\psin \right]
,&\>\>
\mb{b}_2 = \mb{A}_2 \left[\begin{matrix} \mb{x}^\ty{O}_1 - \mb{x}_1 \\ \mb{x}^\ty{O}_2 - \mb{x}_2 \end{matrix}\right].
\label{eq:TaskParametersWithObjectTracking}
\end{align}
%
\subsection{The general case of $N_T$ tasks}
\label{subsec:generalizationNTasks}
The approach can be generalized to the case of $N_T$ arbitrary tasks, framed in the context of TP-GMM. If we consider $N_T$ tasks and $j=1,\hdots,P$ candidate hierarchies, represented by $\mb{A}_j$, \eqref{eq:Task1HierarchyOp} and \eqref{eq:Task2HierarchyOp} are generalized to
%
%\begin{align}
%\left[\begin{matrix} \mb{\hat{\dot{x}}}_1 \\ \vdots \\ \mb{\hat{\dot{x}}}_{N_T} \end{matrix}\right] 
%&= \left[\begin{matrix} \mb{J}_1 \\ \vdots \\ \mb{J}_{N_T} \end{matrix}\right]
%\mathcal{H}_j 
%\left[\begin{matrix} \mb{\dot{x}}_1 \\ \vdots \\\mb{\dot{x}}_{N_T} \end{matrix}\right],
%\label{eq:GeneralizedProjection}
%\end{align}
%
%where $\mathcal{H}_j$ is the candidate task hierarchy matrix $j$, built from arranging the Jacobian pseudo-inverses and null-space projection matrices of the considered tasks. For the previous example, $\mathcal{H}_1 = \mb{A}_1 = \left[\mb{J}_1^\psin \quad \mb{N}_1\mb{J}_2^\psin \right]$ and $\mathcal{H}_2 = \mb{A}_2 = \left[\mb{N}_2\mb{J}_1^\psin \quad \mb{J}_2^\psin \right]$, but this is not always the case. Indeed, $\mathcal{H}_1 \neq \mb{A}_1$ and $\mathcal{H}_2 \neq \mb{A}_2$ if we consider the problem of tracking an object with the different priorities described by \eqref{eq:TaskParametersWithObjectTracking}. 
%
\begin{align}
\left[\begin{matrix} \mb{\hat{\dot{x}}}_1 \\ \vdots \\ \mb{\hat{\dot{x}}}_{N_T} \end{matrix}\right] 
&= \left[\begin{matrix} \mb{J}_{\!1} \\ \vdots \\ \mb{J}_{\!N_T} \end{matrix}\right]
\mb{A}_j 
\left[\begin{matrix} \mb{\dot{x}}_1 \\ \vdots \\\mb{\dot{x}}_{N_T} \end{matrix}\right].
\label{eq:GeneralizedProjection}
\end{align}

Note that one is not required to provide all possible combinations of these matrices for the $N_T$ tasks. The candidate hierarchies can be seen as prior information given by the user, equivalently to the coordinate systems given to TP-GMM in the case of objects of potential interest for the task. In the same way that some objects might be known to be unimportant, some hierarchies may also be known to be irrelevant beforehand. %Equation \eqref{eq:GeneralizedProjection} can then be seen as a local frame projection in the TP-GMM sense \eqref{eq:TPprojection}. In particular, if we make $\mb{\bar{J}}_t=\left[\mb{J}^\trsp_{t,1} \> \hdots \> \mb{J}^\trsp_{t,N_T} \right]^\trsp$ and we consider the datapoint $\mb{\xi}_t = \left[\mb{\dot{x}}^\trsp_{t,1} \> \hdots \> \mb{\dot{x}}^\trsp_{t,N_T} \right]^\trsp$, the local frame projection is obtained according to 
If we use $\mb{\bar{J}}_t=\left[\mb{J}^\trsp_{t,1} \> \hdots \> \mb{J}^\trsp_{t,N_T} \right]^\trsp$ and consider the datapoint $\mb{\xi}_t = \left[\mb{\dot{x}}^\trsp_{t,1} \> \hdots \> \mb{\dot{x}}^\trsp_{t,N_T} \right]^\trsp$, the mapping of the data to a frame $j$, that represents a candidate hierarchy, is obtained according to
%
%\begin{equation}
%\mb{\xi}^{(j)}_t = \mb{\bar{J}}_t\mathcal{H}_{t,j} \mb{\xi}_t
%\label{eq:GeneralizedProjectionFrames}\>.
%\end{equation}
\begin{equation}
\mb{\xi}^{(j)}_t = \mb{\bar{J}}_t\mb{A}_{t,j} \mb{\xi}_t
\label{eq:GeneralizedProjectionFrames}\>.
\end{equation}

A TP-GMM can then be estimated using the same EM algorithm as described in Section \ref{sec:LearningTPMovements}. Movement synthesis is performed through Gaussian product, which is a generalization of \eqref{eq:controllerWeightingStrictHierarchies} for the case of $P$ candidate hierarchies. %, followed by GMR 
Note that, in this type of application, there is a decoupling between the task-parameters that are used for projecting data in the local frames of TP-GMM and those that are used for reproduction. Indeed, the choice of the task-parameters is centered on the desired behavior during reproduction, with the options of choosing those of the type \eqref{eq:TaskParametersNoObject} or \eqref{eq:TaskParametersWithObjectTracking}, while the projection of data is always performed according to \eqref{eq:GeneralizedProjectionFrames} (regardless of the value of $\mb{b}_j$). This is related to the fact that one now uses TP-GMM to encode operational space velocities instead of poses.



==> sections/acknowledgements.tex <==
%\section*{Acknowledgements}
%We would like to thank Luca Muratore and Phil Hudson for assisting with the COMAN experiments and Dr Martijn Zeestraten, Arturo Laurenzi and Giuseppe Rigano for the help with the Centauro simulator. We would also like to thank Dr Yanlong Huang for his feedback on previous versions of the paper.


==> sections/experiments.tex <==
\section{Experiments}%\footnote{Videos of the experimental results are available at http://programming-by-demonstration.org/T-RO\_2016/ }}
\label{sec:expResults}
%We showcase the proposed approach in two distinct scenarios: a bimanual sweeping experiment and a bimanual shaking task. While sweeping requires coordinated task-space movements between the two hands, in particular complex orientation patterns, the shaking skill combines task-space constraints (bottle pose for grasping, opposite end-effector pose for keeping a constant distance and orientation) and joint-space constraints (rhythmic joint movements regardless of where the robot is in task space). Therefore the experiments strongly demonstrate the potential of method.

% JS: removed from the first submission
%\subsection{Learning bimanual coordination in operational space: sweeping task}
%\label{sec:SweepingResults}
%
%We apply the proposed framework to the learning of a bimanual sweeping task, a particular case where bimanual coordination patterns arise, encompassing both position and orientation constraints. Sweeping is a common task whose realization in humanoid robots has been the focus of several developments over the years, see e.g. \cite{Okada06}.
%We employ two torque-controlled 7-DoF Barrett WAM robots, see Fig.\ \ref{Fig:SweepingWAMs}. A broom is attached to the right end-effector using a passive Cardan joint, while the left arm uses a Barrett robotic hand to hold the broom. Since the broom is passively attached to the right arm, the sweeping movement consists of a rotation between the two end-effectors, with the hand grabbing the broom and describing a pendulum-like motion with respect to the end-effector of the right arm.
%
%\begin{figure}
%	%\vspace{-0.1cm}
%	\centering
%	\includegraphics[width=0.8\columnwidth]{figures/Broom}
%    \caption{Two WAM 7-DoF robots performing a bimanual sweeping task. %Bimanual tasks are an example of manipulation tasks where the orientation constraints are at least as important as position constraints (in this figure, the orientation between the end-effectors is crucial to the success of the sweeping task). We propose a method that allows the robots to learn both position and orientation constraints from demonstrations.
%    }
%	\label{Fig:SweepingWAMs}
%\end{figure}
%
%We collected 4 demonstrations with a duration of approximately 8 seconds each through kinesthetic teaching, while the position and orientation of each of the end-effectors were recorded. During the demonstrations, both robots were physically moved with a controller compensating for the effect of gravity. Since unit quaternions provide a double coverage of $SO(3)$ ($\mb{\epsilon}$ and $-\mb{\epsilon}$ represent the same orientation), we pre-process the data to ensure that there is no discontinuity in the demonstrated signals (a mere sign check). During control we also made sure that the quaternion returned by the forward kinematics is the closest quaternion to the reference. In order to learn the movement, we trained the task-parameterized model using $K=10$ Gaussians ($K$ chosen empirically but methods based on a Bayesian information criterion \cite{Schwarz78} could alternatively be used for model selection).
%
%In the experiments described in this section we have used the statistical dynamical system described in Appendix \ref{app:DynamicalSytems}. We used $\mb{K}_p=500 \mb{I}$ and $\mb{K}_v=45 \mb{I}$ to compute the position attractors of the left arm, $\mb{K}_p=250 \mb{I}$ and $\mb{K}_v=35 \mb{I}$ for the right arm and $\mb{K}_o=250 \mb{I}$, $\mb{K}_\omega=35 \mb{I}$ to compute the orientation attractors of both arms (where $\mb{I}\in\mathbb{R}^{3\times3}$). The values of $\mb{K}_v$ and $\mb{K}_\omega$ were chosen empirically by keeping the unit mass-spring-damper system overdamped ($\mb{K}_{v,\omega}>2\sqrt{\mb{K}_{p,o}}$). 
%%A video accompanying this paper shows the results of the experiments, and is available at \texttt{\footnotesize http://programming-by-demonstration.org/iros2015/}. We also provide  Matlab source codes presenting the overall approach described in sections \ref{sec:TPGMM} and \ref{sec:GeneralizedSDS} with a simple example (codes compatible with GNU Octave).
%%The experiments described next can be visualized in the accompanying video, that is also available in \texttt{\footnotesize http://programming-by-demonstration.org/iros2015/}
%
%%\begin{figure}%[htb]
%%	\centering
%%  	\includegraphics[width=\columnwidth]{figures/PositionsALL_tightCrop}
%%% 	\vspace{-0.7cm}
%%     \caption{Time evolution of the position dimensions of both end-effectors during one reproduction attempt, represented in the coordinate system of the area to be swept by the broom. The grey lines show the demonstrated trajectories, the red line shows the position attractor that is output by GMR and the blue line shows the resulting end-effector positions. Time is displayed in seconds and positions in meters.}
%% 	\label{Fig:2frames_AllinOnePos}
%% 	\vspace{-0.5cm}
%%\end{figure}
%
%%\begin{figure*}%[ht]
%%	\centering
%%    \includegraphics[width=\textwidth]{figures/QuaternionsALL_tightCrop}
%%    \caption{Time evolution of the quaternions representing the orientation of each end-effector with respect to the coordinate system of the sweeping area, during one reproduction attempt. Grey lines correspond to the demonstrations, while red and blue lines depict the quaternion attractors (normalized output of GMR) and the retrieved quaternions, respectively.}
%% 	\label{Fig:2frames_AllinOneQuat}
%% 	\vspace{-0.5cm}
%%\end{figure*}
%
%\begin{figure}%[ht]
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figures/QuaternionsALLvertical_tightCrop}
%	\caption{Time evolution of the quaternions representing the orientation of each end-effector with respect to the coordinate system of the sweeping area, during one reproduction attempt. Grey lines correspond to the demonstrations, while red and blue lines depict the quaternion attractors (normalized output of GMR) and the retrieved quaternions, respectively.}
%	\label{Fig:2frames_AllinOneQuat}
%\end{figure}
%
%%\begin{figure*}%[ht]
%%	\centering
%%    \includegraphics[width=\textwidth]{figures/PoseALL_new}
%%    \caption{Time evolution of the quaternions representing the orientation of each end-effector with respect to the coordinate system of the sweeping area, during one reproduction attempt. Grey lines correspond to the demonstrations, while red and blue lines depict the quaternion attractors (normalized output of GMR) and the retrieved quaternions, respectively.}
%% 	\label{Fig:2frames_AllinOneQuat}
%% 	\vspace{-0.5cm}
%%\end{figure*}
%
%\subsubsection*{Encoding bimanual coordination patterns} 
%We encode the task using two frames ($P\!=\!2$), a moving frame ($j\!=\!1$) given for each arm by the coordinate system defined by the position and orientation of the opposite end-effector, and a fixed frame ($j\!=\!2$) defined by the area to be swept by the broom. %Instead of considering two separate TP-GMM (one per arm) we use one single model, for compactness, that includes the 
%We consider task-parameters associated with both end-effectors. Therefore, we define $\mb{\xi}_t$ and $\mb{b}_{t,1},\mb{A}_{t,1}$, the task parameters of frame $j\!=\!1$, as
%\begin{equation*}
%  \!\!\!\mb{\xi}_t\!\!=\!\!\begin{bmatrix} t \\ \mb{\hat{x}}^\mathcal{L}_t \\ \mb{\hat \epsilon}^\mathcal{L}_t \\ \mb{\hat{x}}^\mathcal{R}_t \\ \mb{\hat \epsilon}^\mathcal{R}_t \end{bmatrix} \hspace{-0.3cm}
%  \begin{matrix}
%  \left. \!\right\}\!\mb{\xi}^\ty{I}_t\\
%  \left. \!\!\begin{matrix}\phantom{0}\\\\\\\phantom{0}\end{matrix}\right\}\!\mb{\xi}^\ty{O}_t
%  \end{matrix}
%	\phantom{0}\!\!, \;	
%	  \mb{b}_{t,1}\!\!=\!\!\!\begin{bmatrix} 0 \\
%  			                         \mb{x}^{\mathcal{R}}_t \\
%  			                         \mb{0} \\
%  			                         \mb{x}^{\mathcal{L}}_t \\
%  			                         \mb{0} \end{bmatrix}\!\!, \;
%\mb{A}_{t,1}\!\!=\!\!\begin{bmatrix} 1 & \!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{0} \\
%							     \mb{0} & \!\!\!\mb{R}{}^{\mathcal{R}}_t & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{0} \\
%								 \mb{0} & \!\!\!\mb{0} & \!\!\!\!\!\HLeft{}^{\mathcal{R}}_t & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{0} \\ 
%								 \mb{0} & \!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{R}{}^{\mathcal{L}}_t & \!\!\!\!\!\mb{0} \\
% 								 \mb{0} & \!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\HLeft{}^{\mathcal{L}}_t \\ \end{bmatrix}\!\!,\!\!
%%  \mb{A}_{t,1}\!\!=\!\!\begin{bmatrix} 1 & \!\!\!\mb{0} & \multicolumn{2}{c}{\hspace{-0.3cm}\ldots} & \!\!\!\!\!\mb{0} \\
%%							     \mb{0} & \!\!\!\mb{R}^{\mathcal{R}}_t & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \multirow{2}{*}{\hspace{-0.2cm}\vspace{0.35cm}\vdots} \\
%%								 \multirow{2}{*}{\vspace{0.35cm}\vdots} & \!\!\!\mb{0} & \!\!\!\!\!\HLeft^{\mathcal{R}}_t & \!\!\!\!\!\mb{0} &  \\ 
%%								 & \!\!\!\mb{0} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\mb{R}^{\mathcal{L}}_t & \!\!\!\!\!\mb{0}\\
% %								 \mb{0} & \multicolumn{2}{c}{\hspace{-0.2cm}\ldots} & \!\!\!\!\!\mb{0} & \!\!\!\!\!\HLeft^{\mathcal{L}}_t \\ \end{bmatrix}\!\!,\!\!
%\end{equation*}
%%\begin{equation}
%%	\label{eq:BiManualTPs}			                         
%%  \mb{A}_{t,1}\!\!=\!\!\begin{bmatrix} 1 & \mb{0} & \mb{0} & \mb{0} & \mb{0} \\
%%							     \mb{0} & \mb{R}^{\mathcal{R}}_t & \mb{0} & \mb{0} & \mb{0} \\
%%								 \mb{0} & \mb{0} & \HLeft^{\mathcal{R}}_t & \mb{0} & \mb{0} \\ 
%%								 \mb{0} & \mb{0} & \mb{0} & \mb{R}^{\mathcal{L}}_t & \mb{0} \\
%% 								 \mb{0} & \mb{0} & \mb{0} & \mb{0} & \HLeft^{\mathcal{L}}_t \\ \end{bmatrix}\!\!,
%%\end{equation}
%%
%where the superscripts $\mathcal{L}$ and $\mathcal{R}$ denote the left and right arm respectively, indicating to which arm corresponds each rotation matrix $\mb{R}_t$, Hamilton operator $\HLeft_t$, end-effector position $\mb{x}_t$ and attractors $\mb{\hat{x}}_t$ and $\mb{\hat \epsilon}_t$. In addition, $t$ is a time step and $\mb{0}$ are zero matrices of appropriate dimension.
%
%The frame $j=2$ is given by the position of the point to be swept by the broom on the floor and an orientation corresponding to that of the bases of the robots (which are aligned in our case). We thus have $\mb{b}_{t,2}=\left[0 \hspace*{0.15cm} \mb{x}^{\mathcal{L}}_{sweep} \hspace*{0.001cm}^\trsp \hspace*{0.15cm}  \mb{0}  \hspace*{0.15cm} \mb{x}^{\mathcal{R}}_{sweep}\hspace*{0.001cm}^\trsp \hspace*{0.15cm} \mb{0} \right]^\trsp$ and ${\mb{A}_{t,2}=\mb{I}}$ (where $\mb{I}\in\mathbb{R}^{15\times15}$). Note that this definition of frames remains valid for a wide range of bimanual skills involving adaptation to objects or landmarks. In the first experiment, the values of $\mb{x}^{\mathcal{L}}_{sweep}$ and $\mb{x}^{\mathcal{R}}_{sweep}$ were randomly selected from the demonstration set\footnote{Alternatively, vision or optical tracking systems may be used to obtain the parameters of the area to be swept.}. 
%
%%Figures \ref{Fig:2frames_AllinOnePos} and \ref{Fig:2frames_AllinOneQuat} show the positions and orientations of both end-effectors over time during the reproduction of one sweep, projected on the frame of the area to be swept, together with local representations of the demonstrations. We observe that the proposed approach successfully reproduces both the demonstrated position and orientation profiles.
%
%Figure \ref{Fig:2frames_AllinOneQuat} shows the orientations of both end-effectors over time during the reproduction of one sweep, projected on the frame of the area to be swept, together with local representations of the demonstrations. We observe that the proposed approach successfully reproduces the orientation profiles.
%
%\subsubsection*{The role of the end-effector frames in coordination} 
%As aforementioned, the main advantage of encoding the task in the frame of the other end-effector is that the bimanual coordination patterns underlying the task, both in position and orientation, are encapsulated in the model. In order to provide a practical example of this property, in particular at the level of orientation, we train a new model using $P=1$, that describes the movement only in the frame of the sweeping area. We then compare how both models react to perturbations, in particular how one arm compensates for perturbations applied to the other. Our hypothesis is that the model with $P=2$ should provide a better compensation given that, in addition to the area to be swept, it also takes into consideration the position and orientation constraints between the two end-effectors. We therefore apply a perturbation to the right arm which consists of adding, via the controller, a force and a torque to its end-effector in task space. The force is applied along the negative direction of the $x_2$-axis, while the torque is applied around the $x_3$-axis of the base of the robot.
%
%\subsubsection{Position} Figure \ref{Fig:2framesPositionPerturbation}-\emph{top} shows the applied force and how it affects the $x_2$ coordinate of both end-effectors. In particular, we observe that the perturbation generates a displacement along $x^{\mathcal{R}}_2$ (see the middle plot), for both $P\!=\!1$ (dashed blue line) and $P\!=\!2$ (solid blue line). The effect of this perturbation on the left arm, however, differs between $P\!=\!1$ and $P\!=\!2$ (Fig.\ \ref{Fig:2framesPositionPerturbation}-\emph{bottom}). In the former case, the attractor $\hat{x}^{\mathcal{L}}_2$ keeps its trend during the perturbation, while in the latter, the model compensates the displacement that occurred in $x^{\mathcal{R}}_2$ by shifting the attractor $\hat{x}^{\mathcal{L}}_2$ accordingly.
%%
%\begin{figure}%[h]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/RpositionsPertALL_tightCrop}
%    \caption{Response of the position along $x_2$ of both arms when a force perturbation is applied to the right arm. The first plot depicts the applied force. The middle and bottom plots represent the attractor (red) and retrieved position value (blue) of the right and left arms, respectively. Dashed lines correspond to $P=1$ while solid lines correspond to $P=2$. Time is in seconds, forces are in Newton, and positions are in meters.}
%	\label{Fig:2framesPositionPerturbation}
%\end{figure}
%%
%\subsubsection{Orientation} We begin by computing the sequence of unit quaternions that represent the orientation between the two end-effectors during a reproduction of the task, $\mb{\bar{\epsilon}}^\mathcal{L}_t*\mb{\epsilon}^\mathcal{R}_t$. These quaternions are then converted into Euler angles for a more intuitive interpretation. Figure \ref{Fig:OrientationPerturbation} shows the 3 Euler angles ($\alpha,\beta,\gamma$ for rotations around $x_3,x_2,x_1$, respectively) alongside with the applied torque. We observe that, during the perturbation, the drift in orientation, with respect to the demonstrations, is greater for the model that was trained using only the frame of reference of the area to be swept (dashed line). As in the case of position, the coordination patterns at orientation level are encoded in the model when $P\!=\!2$, resulting in a better reaction to perturbations since the relative orientation is considered by the model.
%
%\begin{figure}%[h]
% 	\centering
%	\includegraphics[width=\columnwidth]{figures/TorqueEuler_tightCrop}
%    \caption{The first plot depicts the task-space perturbation torque that was applied to the end-effector of the right arm. The remaining three plots represent the orientation between the two end-effectors as Euler angles (computed, for visualization purposes, from the quaternions $\mb{\bar{\epsilon}}^\mathcal{L}_t*\mb{\epsilon}^\mathcal{R}_t$ for every $t$). The dashed lines correspond to the model that was trained using $P=1$, while the solid lines correspond to $P=2$. Time is in seconds, torques are in Newton-meter, and angles are in radians.}
%	\label{Fig:OrientationPerturbation}
%\end{figure}
%
%These results show that the proposed learning framework is able to successfully encode and synthesize position and orientation constraints in bimanual manipulation scenarios, by taking advantage of the new structure of the task parameters, described in Section \ref{sec:LearningTPMovements}. In particular, they highlight how encoding the bimanual coordination patterns in the model is essential for a robust execution of the task and how the quaternion-based dynamical systems formulation can reproduce the demonstrated orientation patterns, even when facing perturbations.
%
%%\subsection*{Extrapolation to new orientations}
%%
%%We now test the generalization capabilities of the approach. A new reproduction is performed with a new set of task parameters for the frame of the sweeping area, $j\!=\!2$, in which its position was shifted by 0.28m along the negative direction of $x_1$, bringing it closer to the bases of the robots, and by 0.05m along the positive direction of $x_2$. In addition, the frame was rotated clockwise by 45$^{\circ}$, with respect to $x_3$. Figures \ref{Fig:GeneralizedEulerBaseFrame} and \ref{Fig:GeneralizedEulerSpotFrame} show the Euler angles that represent the orientation of both end-effectors during one reproduction of the sweeping movement using the new frame. The orientations are represented in the coordinate system of the bases of the robots (Fig. \ref{Fig:GeneralizedEulerBaseFrame}) and in the coordinate system of the area to sweep (Fig. \ref{Fig:GeneralizedEulerSpotFrame}). Figure  \ref{Fig:GeneralizedEulerBaseFrame} shows that the values of $\alpha^\mathcal{L}$ and $\alpha^\mathcal{R}$ (rotations around $x_3$), that were retrieved during the reproduction, have an offset of about $0.8rad$ ($\approx$ 45$^{\circ}$) with respect to the demonstrations. Hence, we can conclude that the movement was properly extrapolated to an orientation that was not demonstrated. In addition, as we can see in Fig. \ref{Fig:GeneralizedEulerSpotFrame}, the orientation of both end-effectors represented in the frame of the sweeping area remained consistent with the demonstrations in that frame, confirming that the movement was correctly reproduced.
%%%
%%\begin{figure}%[htb]
%% 	\centering
%%	\includegraphics[width=\columnwidth]{figures/GeneralizationEulerBase_tightCrop}
%%     \caption{The orientation of the end-effectors with respect to the frames of the robot bases (represented in Euler angles) during a reproduction attempt with new task parameters. Blue lines show the retrieved Euler angles, while gray lines show the demonstrations. Angles are in radians and time in seconds.}
%% 	\label{Fig:GeneralizedEulerBaseFrame}
%%\end{figure}
%%\vspace{-0.1cm}
%%\begin{figure}%[htb]
%% 	\centering
%%	\includegraphics[width=\columnwidth]{figures/GeneralizationEulerSpot_tightCrop}
%%     \caption{End-effector orientations, represented in Euler angles, locally represented in the coordinate system of the sweeping area for the new values of the task parameters. The blue lines correspond to the retrieved values during the reproduction, while the demonstrations are depicted in grey. Angles are in radians and time is in seconds.}
%% 	\label{Fig:GeneralizedEulerSpotFrame}
%% 	\vspace{-0.5cm}
%%\end{figure}
% JS: end of remove from first submission

% JS: Moved to the handling constraints section
%\subsection{Learning constraints in operational and configuration spaces: shaking task}
%\label{subsec:shakingTask}
%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{figures/COMAN_fullMove_lowRes}
%%	\includegraphics[width=\columnwidth]{figures/COMAN_fullMove2x2}
%	\caption{The COMAN robot performs the bimanual shaking task in the Gazebo simulator. \textbf{First:} The robot is in a neutral starting pose. \textbf{Second:} Reaching for the bottle and grasping it. \textbf{Third:} Bringing the bottle closer to the torso. \textbf{Fourth:} Shaking movement executed through rhythmic oscillations of both shoulder joints.}
%	\label{fig:COMAN_Shaking}
%\end{figure}
%
%In a second experiment we tested the configuration space projection operators introduced in Section \ref{sec:combiningConstraints}. We selected the skill of shaking a bottle using COMAN. The whole movement contains an operational space component --reaching, grasping a bottle and bringing it closer to the torso-- and a configuration space component --shaking with rhythmic movements of the shoulders (Figure \ref{fig:COMAN_Shaking}).%Such skill combines operational and configuration space constraints: on one hand there are constraints related to the pose of the object to be grasped, bimanual pose constraints, to keep relative poses constant, and a rhythmic joint movement in configuration space that performs the act of shaking, regardless of the end-effector pose in operational space. 
%
%The upper-body of the COMAN robot comprises 17 DOFs (3 DOFs for the waist and 7 for each arm) with the kinematic chains of both arms sharing the waist joints. We define the differential kinematics of the left and right end-effectors using the  \textit{upper-body Jacobian}, $\mb{J}_{\!up}\mb{\dot{q}} = \left[\mb{\dot{x}}^\trsp_L \>\> \mb{\dot{x}}^\trsp_R\right]^\trsp$, as defined by \cite{Lee14}. Here, $\mb{\dot{x}}_L$, $\mb{\dot{x}}_R$ are the left and right end-effector velocities and $\mb{\dot{q}}=\left[\mb{\dot{q}}^\trsp_{W} \>\> \mb{\dot{q}}^\trsp_L \>\> \mb{\dot{q}}^\trsp_R\right]^\trsp$ are the joint velocities of waist, left and right arm joints. The Jacobian matrix is given by
%%
%\begin{equation}
%	\mb{J}_{up} = \left[\begin{matrix}	\mb{J}_{W|L} & \mb{J}_{\!\!L} & \mb{0} \\
%										\mb{J}_{W|R} & \mb{0}   & \mb{J}_{\!\!R}     \end{matrix}\right],
%\end{equation}
%%
%where $\mb{J}_{W|L}$, $\mb{J}_{W|R}$ denote the Jacobians that account for the effect of the waist joints on left and right end-effector velocities. $\mb{J}_{\!\!L}$ and $\mb{J}_{\!\!R}$ correspond to the Jacobians of the left and right end-effectors from the waist link. The least norm inverse kinematics solution is given in this case by ${\mb{\hat{\dot{q}}} = \left[\begin{matrix} \mb{\hat{\dot{q}}}^\trsp_{W} \> \mb{\hat{\dot{q}}}^\trsp_L \> \mb{\hat{\dot{q}}}^\trsp_R \end{matrix}\right]^\trsp \!\!=\! \mb{J}^\psin_{up}\> \left[\begin{matrix} \mb{\hat{\dot{x}}}^\trsp_L \> \mb{\hat{\dot{x}}}^\trsp_R \end{matrix}\right]^\trsp}\!\!$,
%%
%%\begin{equation}
%%	\mb{\hat{\dot{q}}} = \left[\begin{matrix} \mb{\hat{\dot{q}}}_{W} \\ \mb{\hat{\dot{q}}}_L \\ \mb{\hat{\dot{q}}}_R \end{matrix}\right] = \mb{J}^\psin_{up}\> \left[\begin{matrix} \mb{\hat{\dot{x}}}_L \\ \mb{\hat{\dot{x}}}_R \end{matrix}\right],
%%	\label{eq:IKUpperBody}
%%\end{equation}
%%
%where $\mb{J}^\psin_{up}$ is computed as in Section \ref{sec:combiningConstraints}.
%
%The experiment was run in the Gazebo simulator. We generated several demonstrations solving the inverse kinematics for the operational space part of the movement, and sinusoidal references for the rhythmic movement of both shoulder joints  performing the shaking part of the task. End-effector positions and orientations, as well as the joint angles of both kinematic chains, were recorded. We collected 10 demonstrations of the skill, each of them with different poses of the object to be grasped and a duration of approximately 13 seconds. Temporal alignment of the demonstrations was achieved using Dynamic Time Warping \cite{Chiu04}. We used a TP-GMM with $K=10$ components, chosen empirically. For each arm we considered $P=2$ frames: the frame defined by \eqref{eq:Ab_xoTable}, parameterized with the pose of the bottle, and the canonical frame \eqref{eq:Ab_qTable} in order to encode the absolute joint trajectories, which are required to perform the shaking movement. In the former we considered the pseudoinverse of the upper-body Jacobian $\mb{J}^\psin_{up,t}$. $\mb{x}^\ty{O}_t$, $\mb{R}^\ty{O}_t$ and $\mb{\epsilon}^\ty{O}_t$ are the position, rotation matrix, and unit quaternion that represent the pose of the bottle at time step $t$. Figures \ref{fig:endEffectorPosShaking}-\ref{fig:JointsShaking} show the dataset over time\footnote{Due to space limitation we only plot data corresponding to the left arm.}, observed from each frame, together with the Gaussian components obtained after EM. In addition we also plot the references generated by GMR, as seen from both frames (red lines), for a new position and orientation of the bottle. In Figures \ref{fig:endEffectorPosShaking} and \ref{fig:endEffectorOrientShaking} we can see that during the reach and grasp movement, there is a low variability in the demonstrations, both in position and orientation, as the end-effector approaches the bottle. This is successfully encoded by the model, as this aspect of the movement is important for a correct completion of the task. Figure \ref{fig:JointsShaking} shows that, from the beginning of the shaking phase, the shoulder joint exhibits a consistent oscillatory pattern that in this case is modeled by 3 Gaussians. This contrasts with the other joints of the robot, which do not influence the shaking movement.
%
%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figures/endEffectorPosShaking}
%	\caption{End-effector position of the left arm from the perspective of the bottle frame. Black lines represent demonstrations while the red line represents one reproduction of the movement. Ellipses depict the Gaussian components of the model (isocontour of one standard deviation). The shaded areas mark the duration of the reach and grasp phase, and the shaking phase. Notice the low variability in position at the end of the reach and grasp movement.}
%	\label{fig:endEffectorPosShaking}
%\end{figure}
%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figures/endEffectorOrientShaking}
%	\caption{End-effector orientation (as a unit quaternion) of the left arm from the perspective of the bottle frame. Notice the low variability in orientation at the end of the reach and grasp movement.}
%	\label{fig:endEffectorOrientShaking}
%\end{figure}
%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figures/JointsShaking}
%	\caption{Waist joints (pitch and yaw) and shoulder joint of the left arm. Notice the low variability of the shoulder joint during the shaking part of the movement (second shaded area) and how the model captures the shaking pattern encoded in this joint.}
%	\label{fig:JointsShaking}
%\end{figure}
%
%%Figure \ref{fig:ShoulderJointTPGMM} shows the advantage of using TP-GMM for this type of task.
%As we pointed out, when using the projection operators defined in Section \ref{sec:combiningConstraints}, each frame corresponds to a candidate configuration space solution. The weight of each solution is estimated from the demonstrations through Gaussian components with appropriate covariance matrices. During movement synthesis, each frame provides a candidate solution which consists of joint angle references with associated variance. Figure \ref{fig:ShoulderJointTPGMM} shows that the TP-GMM correctly extracted the most relevant solution according to the requirements of the task. Notice how until $t\!\approx\!5s$ TP-GMM matches the candidate solution that corresponds to the bottle frame. Since the variability encoded in this frame is low compared to that of the canonical frame (a consequence of the reach and grasp skill being governed essentially by operational space constraints), the Gaussian product favors this solution. This is achieved through the linear transformation properties of Gaussians, that allow for both centers and covariance matrices to be locally mapped from operational to configuration space using the operators defined in Table \ref{tab:AbOrient}. Similarly, during the shaking phase, after $t\!\approx\!8s$ the reference generated for the shoulder joint matches the estimate from the canonical frame. This is due to the shaking movement resulting in a consistent oscillatory pattern of that joint observed during the demonstrations, as seen in Fig.\ \ref{fig:JointsShaking}. This shows that TP-GMM is a viable solution for the encoding of task relevant features in both operational and configuration spaces. This example shows that this information is essential for movement synthesis in new situations with a proper generalization of the demonstrated skill.
%
%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figures/ShoulderJointTPGMM}
%	\caption{Shoulder joint position estimation from each frame and the resulting reference after TP-GMM. Each estimate has an associated mean and variability, learned from the demonstrations of the movement and regenerated during reproduction. Through Gaussian product, TP-GMM combines the most relevant frames at each time step.}
%	\label{fig:ShoulderJointTPGMM}
%\end{figure}
% JS: End of moved to handling constraints section

\subsection{Learning task priorities with the humanoid robot COMAN}
We now test the hierarchy extraction and synthesis capabilities of our algorithm, described in Section \ref{subsec:priorityConstraints}. Since the kinematic chains of the humanoid arms share the waist joints, task incompatibilities often occur during bimanual manipulation when the tasks of the two arms are too far apart (Fig.\ \ref{fig:COMAN_PrioritiesCloseFar}). %We propose to learn from data which arm should be prioritized in such a situation. We consider the case where there are two references in the workspace of the robot that must be tracked with each of the hands. This scenario is depicted in Figure \ref{fig:COMAN_PrioritiesCloseFar} where the COMAN robot must track a reference position with each hand. In the depicted situation, both tasks have the same priority and therefore, when new references are incompatible (i.e., the two cannot be reached simultaneously) the robot does not fulfill any of the tasks.
We propose to demonstrate which of the arms has priority over the other and learn that priority using TP-GMM. If the priority is correctly learned, the robot will track both references when both are reachable, and prioritize one of them when the two become incompatible.

We consider a TP-GMM with $P=2$ candidate hierarchies, corresponding to the two possible combinations of priority, i.e. priority on left arm with the right arm as secondary and vice-versa. We denote the Jacobians of each arm (from the base link) by $\mb{J}_{\!\!L}$, $\mb{J}_{\!\!R}$, their pseudoinverses by $\mb{J}^\psin_{\!\!L}$, $\mb{J}^\psin_{\!\!R}$ and the null-space projection matrices by $\mb{N}_{\!\!L}$, $\mb{N}_{\!\!R}$. 
%We thus consider the two candidate hierarchy matrices
%%
%\begin{equation}
%	\mathcal{H}_1 = \left[\mb{J}^\psin_L \>\> \mb{N}_L\mb{J}^\psin_R \right], \quad
%	\mathcal{H}_2 = \left[\mb{J}^\psin_R \>\> \mb{N}_R\mb{J}^\psin_L \right]. 
%	\label{eq:candidateHierachiesBimanual}
%\end{equation}
We thus employ the task parameters
%
\begin{align}
\mb{A}_1 = \left[\mb{J}^\psin_{\!\!L} \>\>\> \mb{N}_{\!\!L}\mb{J}^\psin_{\!\!R} \right]
,&\qquad
\mb{b}_1 = \mb{A}_1 \left[\begin{matrix} \mb{x}^\ty{O}_L - \mb{x}_L \\ \mb{x}^\ty{O}_R - \mb{x}_R \end{matrix}\right]
,\nonumber\\
\mb{A}_2 = \left[\mb{N}_{\!\!R}\mb{J}^\psin_{\!\!L} \>\>\> \mb{J}^\psin_{\!\!R} \right]
,&\qquad
\mb{b}_2 = \mb{A}_2 \left[\begin{matrix} \mb{x}^\ty{O}_L - \mb{x}_L \\ \mb{x}^\ty{O}_R - \mb{x}_R \end{matrix}\right],
\label{eq:TPsWithObjectTrackingBimanual}
\end{align}
%%
%\begin{equation}
%\mathcal{H}_1 = \left[\mb{J}^\psin_L \>\> \mb{N}_L\mb{J}^\psin_R \right], \quad
%\mathcal{H}_2 = \left[\mb{J}^\psin_L \>\> \mb{N}_L\mb{J}^\psin_R \right],. 
%\label{eq:candidateHierachiesBimanual}
%\end{equation}
%%
where $\mb{x}^\ty{O}_L$ and $\mb{x}^\ty{O}_R$ denote left and right reference positions.
In addition, we use datapoints of the form $\mb{\xi}_t = \left[\begin{matrix} \mb{e}^\trsp_{L,t} \>\> \mb{e}^\trsp_{R,t}\end{matrix}\right]^\trsp \in \mathbb{R}^6$, where $\mb{e}^\trsp_{L,t}, \mb{e}^\trsp_{R,t}$ are the tracking errors of left and right arm tasks during demonstrations.
%For matrices \eqref{eq:candidateHierachiesBimanual}, and since we consider the problem of tracking an object, the task parameters follow from \eqref{eq:TaskParametersWithObjectTracking}:
%%
%\begin{align}
%	\mb{A}_1 = \mathcal{H}_1
%	,&\qquad
%	\mb{b}_1 = \mathcal{H}_1 \left[\begin{matrix} \mb{x}^\ty{O}_L - \mb{x}_L \\ \mb{x}^\ty{O}_R - \mb{x}_R \end{matrix}\right]
%	,\nonumber\\
%	\mb{A}_2 = \mathcal{H}_2 
%	,&\qquad
%	\mb{b}_2 = \mathcal{H}_2 \left[\begin{matrix} \mb{x}^\ty{O}_L - \mb{x}_L \\ \mb{x}^\ty{O}_R - \mb{x}_R \end{matrix}\right],
%	\label{eq:TPsWithObjectTrackingBimanual}
%\end{align}
%
%where $\mb{x}^\ty{O}_L$, $\mb{x}^\ty{O}_R$ denote left and right reference positions, and $\mb{R}^\ty{O} = \mb{I}$ since we do not consider the tracking of orientation.
We used for this task $K=1$ (same hierarchy throughout the task, selected empirically). %By using a GMM we could have time-varying priorities on each hierarchy but this way we show that with a model as simple as a single multivariate Gaussian we can already encode complex behavior.

Demonstrations of the priorities were provided by implementing an inverse kinematics solution with the desired hierarchy in the simulated robot and making it track moving references\footnote{Alternatively, kinesthetic teaching or optical tracking of movements from humans could also be used, by recording the tracking errors as well as the kinematic data of the demonstrator (that would allow for computing the Jacobians required for the projections of observed movements).}. Since the estimation of the hierarchy structure is based on the tracking error, a single demonstration contains sufficient datapoints for a correct model to be learned, provided that the priority behavior is shown, namely, that one of the arms cannot fulfill its task while the other can.
% -- The below part was used when considering the 3D plots of the projected data --
%For the case of priority on the left arm we obtained the dataset shown in Figure \ref{fig:LeftPriorityDataSet}. In this figure, we can observe that the projected data according to the candidate hierarchies results in a low variability for the hierarchy whose most important task is the tracking of the left object. Figure \ref{fig:RightPriorityDataSet} shows equivalent results for the case when the robot is controlled with a priority on the right arm.
We generated demonstrations of the two different possibilities of priority for this setup and analyzed the resulting datasets. Figure \ref{fig:PriorityDataSets} shows the tracking errors of each hand after applying \eqref{eq:GeneralizedProjection} with the task parameters \eqref{eq:TPsWithObjectTrackingBimanual}. %We observe that the projected data according to the candidate hierarchies results in a low variability for the hierarchy that was demonstrated.
We observe negligible, invariant errors for the hierarchies that were demonstrated.

Low variability results in high precision matrices $\mb{\Gamma}$, which in turn, during movement synthesis, results in higher weights being assigned to the hierarchies with low variability. We applied the learned models in both the left- and right-priority scenarios to reach fixed points on the left and right sides of the robot, with the results depicted in Fig.\ \ref{fig:COMANPriority}. %Figures \ref{fig:COMANPriorityLeft} and \ref{fig:COMANPriorityRight}
As expected, in both cases, we observe that the arm having the highest priority in the demonstrated movement is always fulfilings the task, while the other only does it when the reference is at a reachable distance.

Similarly to the example in Section \ref{subsec:shakingTask}, each candidate hierarchy provides a candidate configuration space solution for the robot. In the particular case of humanoid robots performing a bimanual skill, the solutions differ in how the waist joints are prioritized (since they are shared by the two arms). Figure \ref{fig:COMAN_WaistJointsLeft} shows the candidate solution given by each frame for the roll, pitch and yaw joints of the waist, during the task of tracking the left object with higher priority. We see that the solution given by the frame that encodes priority on the left arm has much lower variability than the one that prioritizes the right tracking task. This leads to a TP-GMM automatically extracting this prioritization as the important one.
%
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/COMAN_EqualPriorityCloseFar}
	\caption{The COMAN robot in the rviz simulation environment performing a bimanual reaching task. \textbf{Left:} Both targets are within the reachable workspace of both arms, so that the robot can successfully reach the centers of the spheres with the palm of its hands. \textbf{Right:} The references moved beyond the part of the workspace where both are reachable at the same time, so that the robot cannot reach any of the two.}
	\label{fig:COMAN_PrioritiesCloseFar}
\end{figure}
%
\begin{figure}%[h]
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=1.0\columnwidth]{figures/LeftPriorityDataSet_points}
		\caption{Demonstrated left-arm priority.}
		\label{fig:PriorityDataSetsLeftArm}
	\end{subfigure}
	\begin{subfigure}{0.49\columnwidth}
		\centering
		\includegraphics[width=1.0\columnwidth]{figures/RightPriorityDataSet_points}
		\caption{Demonstrated right-arm priority.}
		\label{fig:PriorityDataSetsRightArm}
	\end{subfigure}
	\vspace{0.3cm}
	\caption{Datapoints obtained through projection of the tracking errors using \eqref{eq:GeneralizedProjection} with task parameters \eqref{eq:TPsWithObjectTrackingBimanual}. %Each color corresponds to a candidate hierarchy projection.
	For better visualization we plot the norm of each hand's error, instead of the 3D points that were used to learn the priority models. The cross represents the mean error. 
%and we omit the error bars since the norm is always positive. 
Notice the low variability in the data corresponding to the demonstrated hierarchies, and the error close to zero (even for the arm with lowest priority).}
	\label{fig:PriorityDataSets}
\end{figure}
%
%\begin{figure}%[h]
%	\centering
%		\includegraphics[width=\columnwidth]{figures/RightPriorityDataSet}
%	\caption{Datapoints and Gaussian of demonstrated priority on the right arm, obtained through projection \eqref{eq:GeneralizedProjection}. Notice, in this case, the low variability of the data corresponding to priority on the right hand.}
%	\label{fig:RightPriorityDataSet}
%\end{figure}
%
%\begin{figure}%[h]
%	\centering
%	\includegraphics[width=0.75\columnwidth]{figures/COMAN_priorityLeft}
%	\caption{Generation of new movements using the left arm priority model that was learned from demonstrations. The left arm task is always fulfilled, while the right arm task is successful when the target is close enough.}
%	\label{fig:COMANPriorityLeft}
%\end{figure}
%%
%\begin{figure}%[h]
%	\centering
%	\includegraphics[width=0.75\columnwidth]{figures/COMAN_priorityRight}
%	\caption{Generation of new movements using the right arm priority model that was learned from demonstrations. The right arm task is always fulfilled, while the left arm task is successful when the target is close enough.}
%	\label{fig:COMANPriorityRight}
%\end{figure}
%%
\begin{figure}%[h]
	\centering
	\includegraphics[width=0.49\columnwidth]{figures/COMAN_priorityLeft}
	\includegraphics[width=0.49\columnwidth]{figures/COMAN_priorityRight}
	\caption{Generation of new movements using the left and right arm priority models that were learned from demonstrations. The main task is always fulfilled, while the secondary task is successful when the target is close enough.}
	\label{fig:COMANPriority}
\end{figure}
%
\begin{figure}%[h]
	\centering
	\includegraphics[width=\columnwidth]{figures/LeftPriorityWaistJoints}
	\caption{Candidate inverse kinematics solutions given by each candidate frame. The envelope around the lines represents the variability encoded in the frames for each joint. The solution proposed by the frame that encodes left-hand priority shows low variability.}
	\label{fig:COMAN_WaistJointsLeft}
\end{figure}
%
%\begin{figure}%[h]
%	\centering
%	\includegraphics[width=\columnwidth]{figures/RightPriorityWaistJoints}
%	\caption{Candidate solutions of the inverse kinematics problem given by each candidate frame. The solution proposed by the frame that encodes priority on the left hand shows much lower variability, which is extracted by TP-GMM during Gaussian product.}
%	\label{fig:COMAN_WaistJointsLeft}
%\end{figure}


\subsection*{Transferring priority constraints between robots}
Since the projections of the data occur in operational space, priority models can be transferred across robots with similar embodiments. We use the model that was learned with COMAN to synthesize an equivalent prioritization behavior in the WALKMAN robot that has a different kinematic structure. WALKMAN is a humanoid larger than COMAN, that also shares the waist joints between the two arms. %Figures \ref{fig:WALKMANPriorityLeft} and \ref{fig:WALKMANPriorityRight}
Figure \ref{fig:WALKMANPriority} shows that the model that was learned using COMAN's kinematic data was successful in generalizing the learned task priorities in WALKMAN. This opens up an interesting strategy to cope with the correspondence problem in imitation learning.
%possibility which is that learned priority models might have a low dependence on the kinematic model of the demonstrator. 
In particular, it could be used by the robot to visually observe a task prioritization behavior demonstrated by the user without explicit direct mapping of the kinematics.

%\begin{figure}%[h]
%	\centering
%	\includegraphics[width=0.75\columnwidth]{figures/WALKMAN_priorityLeft}
%	\caption{Movement synthesis with the WALKMAN robot using the left-priority model that was learned with COMAN.}
%	\label{fig:WALKMANPriorityLeft}
%\end{figure}
%%
%\begin{figure}%[h]
%	\centering
%	\includegraphics[width=0.75\columnwidth]{figures/WALKMAN_PriorityRight}
%		\caption{Movement synthesis with the WALKMAN robot using the right-priority model that was learned with COMAN.}
%	\label{fig:WALKMANPriorityRight}
%\end{figure}
\begin{figure}%[h]
	\centering
	\includegraphics[width=0.49\columnwidth]{figures/WALKMAN_priorityLeft_lowRes}
	\includegraphics[width=0.49\columnwidth]{figures/WALKMAN_PriorityRight_lowRes}
	\caption{Movement synthesis with the WALKMAN robot using the left and right priority models that were learned with COMAN.}
	\label{fig:WALKMANPriority}
\end{figure}
%
\subsection{Soft weighting of hierarchies: behavior during transitions}
%
An important aspect to consider when controlling priorities is the behavior of the robot when priorities change. In order to investigate how our approach performs in such cases, we study in this section the effect of varying the weights of each candidate hierarchy. For simplicity of analysis, we consider the case of a planar robot with two tasks, similar to the example in Section \ref{subsec:priorityConstraints}. The tasks are to track a vertical position reference with the end-effector and to point downwards. The references are chosen such that the two tasks can be fulfilled individually but not simultaneously (Fig.\ \ref{fig:VariableWeights}, \emph{top-left}). Two strict hierarchies are considered, corresponding to an accurate tracking of either position or orientation as first priority, and orientation or position as secondary. We define two scalar weights $w_{\text{pos}}$ and $w_{\text{orient}}$, which represent the importance of each hierarchy, with the subscript denoting the highest priority task. These weights are used to compute the precision matrices $\mb{\Gamma}_{\text{pos}} \!=\! w_{\text{pos}}\mb{I}$ and $\mb{\Gamma}_{\text{orient}} \!=\! w_{\text{orient}}\mb{I}$,
%
%\begin{equation}
%	\mb{\Gamma}_{\text{pos}} = w_{\text{pos}}\mb{I}, \qquad	\mb{\Gamma}_{\text{orient}} = w_{\text{orient}}\mb{I},
%\end{equation}
%
where $\mb{I}$ is a 2-dimensional identity matrix. Figure \ref{fig:VariableWeights} shows the results for the case in which the robot transits from the orientation to the position tracking task, through a continuous variation of the weights. We observe that, as different combinations of weights are applied by the controller, a smooth transition occurs between the two tasks. 

%\begin{figure}
%	\centering
%	\includegraphics[width=0.49\columnwidth]{figures/PlanarRobotTrackPos}
%	\includegraphics[width=0.49\columnwidth]{figures/PlanarRobotTrackOrient}
%	\caption{A 3-DOF planar robot performing two different tasks: reaching a desired vertical position with its end-effector while staying on the horizontal line, and maintaining a desired orientation (indicated by the arrow). When performing one of the tasks, it tries to fulfill the other as best as possible. In some configurations, the two tasks are incompatible, i.e., they cannot be completed simultaneously, but can be achieved individually.
%		}
%	\label{fig:PlanarRobotTasks}
%\end{figure}

 \begin{figure}
 	\centering	
% 	\includegraphics[width=\columnwidth]{figures/VariableWeightPlots}
  	\includegraphics[width=\columnwidth]{figures/variableWeightsAllinOne}
 	\caption{End-effector behavior for varying hierarchy weights. \textbf{Top-left:} Planar robot fulfilling the two tasks separately. \textbf{Top-right:} End-effector state in the position-orientation space for the considered weights (blue line). \textbf{Bottom:} End-effector orientation and vertical position as weights vary. Notice the inverted scales on the horizontal axes - the experiment starts with $(1,0)$ and ends with $(0,1)$. Red lines and point indicate the references.}
 	\label{fig:VariableWeights}
 \end{figure}

Another case that is worth investigating is the behavior of the system when both tasks are achievable. In this situation one would expect that any combination of the weights would result in a successful completion of both tasks. In order to test how our approach handles this scenario, we decreased the vertical position reference so that both tasks can be fulfilled simultaneously. % (Figure \ref{fig:PlanarRobotFeasibleTasks}).
We set the robot to an initial configuration $\mb{q}_{\text{init}} = [\frac{\pi}{2}\!+\!0.5, \>\> -1, \>\> -\frac{\pi}{2}\!+\!0.5]$. %and tested two distinct situations. First, 
The robot is initialized to that configuration and, for every new pair of weights, its starting configuration is that of the previous pair. % to which it converged with
%In the second situation, the configuration is reset to $\mb{q}_{\text{init}}$ for every new pair of weights. 
Figure \ref{fig:PlanarRobotPerformanceFeasible} shows the tracking performance. %, where we used 40 time steps of simulation per weight pair. 
We can see that the observed end-effector pose tracked the reference with a negligible error. %, see Figure \ref{fig:PlanarRobotFeasibleTasks}. 
%The illustration in Figure \ref{fig:PlanarRobotFeasibleTasks}-\emph{left} corresponds to this situation. 
This result shows that the approach converges to a proper solution and maintains it when the weights are modified. In other words, once the robot converged to a configuration that fulfills both tasks, with the initial weights $(w_{\text{orient}},w_{\text{pos}}) = (1,0)$, further variations of the weights did not affect the solution, as one would expect. 
%Figure \ref{fig:PlanarRobotPerformanceFeasibleReInit} shows the performance results for the second scenario that we considered, i.e., when the configuration of the robot is reset for each pair of weights. The top plots show the tracking performance for 40 time steps per weight pair. The graphs show a performance degradation with respect to the previous case, with errors greater than $0.02$rad and  $0.02$m. Figure \ref{fig:PlanarRobotFeasibleTasks}-\emph{right} shows the configuration of the robot for some of the weight pairs in this situation. This is somewhat unexpected, since both tasks can be achieved, so the weight variations should not affect the solution. The bottom plots in Figure \ref{fig:PlanarRobotPerformanceFeasibleReInit} were obtained from re-running the simulation with the same references but increasing the number of steps to 250. As we can see, this resulted in a considerable decrease in the observed tracking errors. This observation suggests that, when starting the robot from a configuration that does not satisfy the task constraints, the method takes longer to converge to a solution that fulfills both tasks. This can be explained by the fact that each candidate hierarchy provides different solutions to the inverse kinematics problem. Since the solutions are in configuration space, even if, individually, they fulfill both tasks, their combination may result in an end-effector pose that does not. For this reason, the robot needs additional time for both frames to converge to a common solution, for any given weight combination.

%These results indicate that changing the priorities between two tasks using our approach is more efficiently done, i.e. faster and less error prone, when both are already fulfilled within a hierarchy. For example, if one wanted to change priorities between arms in the bimanual tracking case, and the robot had its priority on the left arm, the transition would occur faster and more smoothly if both targets were within the reach of the robot.

%\begin{figure}
%	\centering
%	\includegraphics[width=0.49\columnwidth]{figures/PlanarRobotBothTasks.jpg}
%	%\includegraphics[width=0.49\columnwidth]{figures/PlanarRobotBothTasksError.jpg}
%	\caption{New position reference allows for both tasks to be fulfilled simultaneously, where %\textbf{Left:} 
%	both tasks are achieved for every combination of priority weights. %\textbf{Right:} The tasks are not achieved for some weight pairs.
%	}
%	\label{fig:PlanarRobotFeasibleTasks}
%\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/PlanarRobotTrackingPerfCase1}
	\caption{Performance of the robot in tracking position and orientation references with varying weights when both tasks can be achieved. Red lines and point indicate the references. % when the initial configuration of the robot is not reset for every new pair of weights.
	}
	\label{fig:PlanarRobotPerformanceFeasible}
\end{figure}

%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{figures/PlanarRobotTrackingErrorsCase2LowNsteps}
%	\\
%	\$ vspace ${0.2cm}
%	\includegraphics[width=\columnwidth]{figures/PlanarRobotTrackingErrorsCase2HighNsteps}
%	\caption{Tracking performance of the robot when its configuration is reset for every weight pair. \textbf{Top:} Errors for  40 time step simulations per weight pair. \textbf{Bottom:} Errors when 250 time steps are used.}
%	\label{fig:PlanarRobotPerformanceFeasibleReInit}
%\end{figure}

Videos of the experiments can be found at  \begin{footnotesize}\texttt{http://joaosilverio.weebly.com/videos}\end{footnotesize}. % other size won't fit in one single line.

